Feature exploration for almost zero-resource ASR-free keyword spotting using a multilingual bottleneck extractor and correspondence autoencoders

We compare features for dynamic time warping (DTW) when used to bootstrap keyword spotting (KWS) in an almost zero-resource setting. Such quickly-deployable systems aim to support United Nations (UN) humanitarian relief efforts in parts of Africa with severely under-resourced languages. Our objective is to identify acoustic features that provide acceptable KWS performance in such environments. As supervised resource, we restrict ourselves to a small, easily acquired and independently compiled set of isolated keywords. For feature extraction, a multilingual bottleneck feature (BNF) extractor, trained on well-resourced out-of-domain languages, is integrated with a correspondence autoencoder (CAE) trained on extremely sparse in-domain data. On their own, BNFs and CAE features are shown to achieve a more than 2% absolute performance improvement over baseline MFCCs. However, by using BNFs as input to the CAE, even better performance is achieved, with a more than 11% absolute improvement in ROC AUC over MFCCs and more than twice as many top-10 retrievals for two evaluated languages, English and Luganda. We conclude that integrating BNFs with the CAE allows both large out-of-domain and sparse in-domain resources to be exploited for improved ASR-free keyword spotting.

==> results_table_luganda.tex <==
% All CAE results here were done with 39-dimesional extracted features.
% Results table that show the test set evaluations that were performed on the full set of keywords.
% In the full set, keywords that occurred less than ten times in the test set were also evaluated.
\begin{table*}[!t]
\caption{
Luganda keyword spotting performance on development and test data using the different feature representations.
Subscripts are in the column headings to distinguish whether MFCCs or BNFs were used as inputs to the AE and CAE.
}
\label{tab:luganda_results39}
\centering
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\parbox{\widthof{Metric}}{\textbf{\vspace{-1ex}Metric}}} & \multicolumn{6}{c}{\textit{{Development} (\%)}} & \multicolumn{4}{c}{\textit{{Test}} (\%)} \\
\cmidrule(lr){2-7} \cmidrule(l){8-11}
& \textbf{MFCC} & \textbf{AE}$_\textrm{\textbf{MFCC}}$ & \textbf{CAE}$_\textrm{\textbf{MFCC}}$ & \textbf{BNF} & \textbf{AE}$_\textrm{\textbf{BNF}}$ & \textbf{CAE}$_\textrm{\textbf{BNF}}$ & \textbf{MFCC} & \textbf{CAE}$_\textrm{\textbf{MFCC}}$ & \textbf{BNF} & \textbf{CAE}$_\textrm{\textbf{BNF}}$ \\
\midrule
AUC     & 66.51 & 67.52 & 69.62 &           71.24             & 72.73 & 78.09 & 69.57 & 69.74 & 73.33 & 80.59 \\
EER     & 38.68 & 38.57 & 37.20 &           33.26             & 31.20 & 29.33 & 37.20 & 37.24 & 33.73 & 29.00 \\
$P$@10  & 11.43 & 14.29 & 28.57 &           11.43             & 10.00 & 45.71 & 18.89 & 27.78 & 26.11 & 41.67 \\
$P$@$N$ & 10.72 & 10.13 & 13.95 & \leavevmode\hphantom{0}9.99 & 11.61 & 26.11 & 13.87 & 18.77 & 18.21 & 28.80 \\
\bottomrule
\end{tabular}
\end{table*}



% All CAE results here were done with 100-dimesional extracted features.
% Results table that show the test set evaluations that were performed on the full set of keywords.
% In the full set, keywords that occurred less than ten times in the test set were also evaluated.
%\begin{table*}[!t]
%\caption{
%Luganda keyword spotting performance on development and test data using the different feature representations.
%Subscripts are in the column headings to distinguish whether MFCCs or BNFs were used as inputs to the AE and CAE.
%}
%\label{tab:luganda_results100}
%\centering
%\begin{tabular}{lcccccccccc}
%\toprule
%\multirow{2}{*}{\parbox{\widthof{Metric}}{\textbf{\vspace{-1ex}Metric}}} & \multicolumn{6}{c}{\textit{{Development} (\%)}} & \multicolumn{4}{c}{\textit{{Test}} (\%)} \\
%\cmidrule(lr){2-7} \cmidrule(l){8-11}
%& \textbf{MFCC} & \textbf{AE}$_\textrm{\textbf{MFCC}}$ & \textbf{CAE}$_\textrm{\textbf{MFCC}}$ & \textbf{BNF} & \textbf{AE}$_\textrm{\textbf{BNF}}$ & \textbf{CAE}$_\textrm{\textbf{BNF}}$ & \textbf{MFCC} & \textbf{CAE}$_\textrm{\textbf{MFCC}}$ & \textbf{BNF} & \textbf{CAE}$_\textrm{\textbf{BNF}}$ \\
%\midrule
%AUC     & 66.51 & -- & 67.35 & 71.24 & -- & 77.72 & 69.57 & 67.63 & 73.33 & 79.00\\
%EER     & 38.68 & -- & 38.37 & 33.26 & -- & 28.80 & 37.20 & 38.90 & 33.73 & 28.38 \\
%$P$@10  & 11.43 & -- & 14.29 & 11.43 & -- & 45.71 & 18.89 & 23.33 & 26.11 & 38.89 \\
%$P$@$N$ & 10.72 & -- & 11.93 & \leavevmode\hphantom{0}9.99 & -- & 26.79 & 13.87 & 15.37 & 18.21 & 25.73 \\
%\bottomrule
%\end{tabular}
%\end{table*}


% Results table that show the test set evaluations that were performed using the reduced set of keywords.
% The reduced set omitted keywords which occurred less than ten times in the test set.
%\begin{table*}[!t]
%\caption{
%Luganda keyword spotting performance on development and test data using the different feature representations.
%Subscripts are in the column headings to distinguish whether MFCCs or BNFs were used as inputs to the AE and CAE.
%% listed in Section~\ref{sec:exp_setup}. All results are reported for the development set but only the baseline MFCC features and best feature representations results are reported for the test set.
%}
%\label{tab:luganda_results100_reduced_keywords}
%\centering
%\begin{tabular}{lcccccccccc}
%\toprule
%\multirow{2}{*}{\parbox{\widthof{Metric}}{\textbf{\vspace{-1ex}Metric}}} & \multicolumn{6}{c}{\textit{{Development} (\%)}} & \multicolumn{4}{c}{\textit{{Test}} (\%)} \\
%\cmidrule(lr){2-7} \cmidrule(l){8-11}
%& \textbf{MFCC} & \textbf{AE}$_\textrm{\textbf{MFCC}}$ & \textbf{CAE}$_\textrm{\textbf{MFCC}}$ & \textbf{BNF} & \textbf{AE}$_\textrm{\textbf{BNF}}$ & \textbf{CAE}$_\textrm{\textbf{BNF}}$ & \textbf{MFCC} & \textbf{CAE}$_\textrm{\textbf{MFCC}}$ & \textbf{BNF} & \textbf{CAE}$_\textrm{\textbf{BNF}}$ \\
%\midrule
%AUC     & 66.51 & -- & 67.35 & 71.24 & -- & 77.72 & 67.61 & 68.64 & 73.64 & 79.04 \\
%EER     & 38.68 & -- & 38.37 & 33.26 & -- & 28.80 & 38.88 & 37.45 & 32.85 & 27.51 \\
%$P$@10  & 11.43 & -- & 14.29 & 11.43 & -- & 45.71 & 26.67 & 32.50 & 36.67 & 51.67 \\
%$P$@$N$ & 10.72 & -- & 11.93 & \leavevmode\hphantom{0}9.99 & -- & 26.79 & 16.43 & 18.68 & 25.71 & 30.03 \\
%\bottomrule
%\end{tabular}
%\end{table*}

